Sign language segmentation with temporal convolutional networks

The objective of this work is to determine the location of temporal boundaries between signs in continuous sign language videos. Our approach employs 3D convolutional neural network representations with iterative temporal segment refinement to resolve ambiguities between sign boundary cues. We demonstrate the effectiveness of our approach on the BSLCORPUS, PHOENIX14 and BSL-1K datasets, showing considerable improvement over the prior state of the art and the ability to generalise to new signers, languages and domains.

==> extra.tex <==

% \noindent - Amount of data: Plot performance against training size. (can skip)\\
% \noindent - Loss formulation: Classification vs regression. (can skip) \\
% \noindent - Iterative refining: regressing to the residual. (can skip) \\
% \noindent - Reduce the effect of dilation. (can skip)

\noindent\textbf{Squeeze-and-Excitation blocks in the architecture.} Through the insertion of a Squeeze-and-Excitation (SE) Layer in each stage of MS-TCN, the sign segment scores improve while the boundary score remains the same (see Tab.~\ref{tab:se}).

\begin{table}
    \centering
    \resizebox{0.75\linewidth}{!}{
    \begin{tabular}{lccc}
         \toprule
         & F1B & F1S@0.75 & IoU  \\
         \midrule
         \methodName{} & 79.38 & 26.97 & 53.90 \\
         \methodName{}+SE & 79.28 & 28.05 & 55.24 \\
         \bottomrule
    \end{tabular}
    }
    \caption{Architectural improvement over MS-TCN.}
    \label{tab:se}
\end{table}

\noindent\textbf{Multi-cue fusion.} In Tab.~\ref{tab:fusion},
we combine pose-based features with the I3D video features.


\begin{table}
    \centering
    \begin{tabular}{lccc}
         \toprule
         & F1B & F1@0.75 & IoU \\
         \midrule
         Geo. & \hmark{} & \hmark{} & \hmark{} \\
         I3D & \hmark{} & \hmark{} & \hmark{} \\
         \midrule
         Geo. + I3D (early) & 78.08 & 27.72 & 55.63 \\
         Geo. + I3D (early) SE & 78.55 & 26.69 & 53.45 \\
         Geo. + I3D (late) & 78.98 & 26.54 & 56.52\\
         Geo. + I3D (late) SE & 76.42 & 29.48 & 57.70\\
         \bottomrule
    \end{tabular}
    \caption{Fusion of I3D and geometric features: (i) early fusion that inputs concatenated features as input to MS-TCN, and (ii) late fusion that averages class probabilities of two separate MS-TCN networks.}
    \label{tab:fusion}
\end{table}

\color{teal}
\section{Weaknesses and Comments}

\begin{enumerate}
    \item The dissonance between the two metrics is quite confusing---it's not clear yet what optimises for F1B (for example, should we add further stages to MS-TCN)? Understanding this is probably our highest priority.
    \item If vanilla MS-TCN ends up outperforming SE layers, we can't claim a new architecture (so we should re-title) and reduce these claims.
    \item We exclude a comparison to the HMM work of Koller et al.~\cite{koller2017re}, but almost all our results make use of semantic labels on \bslcorpus{} and \bslonek{}.  We could claim something about annotation sparsity if needed.
    \item Further thoughts: (i) there may still be a significant capacity issue if increasing the number of feature maps brings a large boost. (ii) if we don't have it yet, I would also try adding batch norm.
    \item Might remove the 25\% number  - perhaps we could then aim for something quantitative with Neil's help for CVPR.
    \item Fusion ...
\end{enumerate}

\color{black}
